Advancing Solutions for the Three-Body Problem Through Physics-Informed Neural Networks

First formulated by Sir Isaac Newton in his work "Philosophiae Naturalis Principia Mathematica", the concept of the Three-Body Problem was put forth as a study of the motion of the three celestial bodies within the Earth-Sun-Moon system. In a generalized definition, it seeks to predict the motion for an isolated system composed of three point masses freely interacting under Newton's law of universal attraction. This proves to be analogous to a multitude of interactions between celestial bodies, and thus, the problem finds applicability within the studies of celestial mechanics. Despite numerous attempts by renowned physicists to solve it throughout the last three centuries, no general closed-form solutions have been reached due to its inherently chaotic nature for most initial conditions. Current state-of-the-art solutions are based on two approaches, either numerical high-precision integration or machine learning-based. Notwithstanding the breakthroughs of neural networks, these present a significant limitation, which is their ignorance of any prior knowledge of the chaotic systems presented. Thus, in this work, we propose a novel method that utilizes Physics-Informed Neural Networks (PINNs). These deep neural networks are able to incorporate any prior system knowledge expressible as an Ordinary Differential Equation (ODE) into their learning processes as a regularizing agent. Our findings showcase that PINNs surpass current state-of-the-art machine learning methods with comparable prediction quality. Despite a better prediction quality, the usability of numerical integrators suffers due to their prohibitively high computational cost. These findings confirm that PINNs are both effective and time-efficient open-form solvers of the Three-Body Problem that capitalize on the extensive knowledge we hold of classical mechanics.

==> 4-methods-and-data_save.tex <==
\section{Methods and Data}
    \label{sec:methods-and-data}

    \subsection{Dataset}
    \label{subsec:data}

    In order to train our models for trajectory prediction, we created a dataset with representative and diverse trajectories that was used to train and validate our model.

    The dataset's generation methodology mirrors that of \citet{Breen2020}, which involves locking the position of a single particle, randomizing the second's position inside some constraints, and obtaining the third by a linear combination of the first two particles' positions.
    Figure~\ref{fig:reference_plane} shows a representation of this process and how each particle is obtained.

    \begin{figure}[h]
        \centering
        \includegraphics[width=\linewidth]{reference_plane}
        \caption{Illustration of the particle's reference plane. Particle $x_1$ is always in the same starting position $\left(1, 0\right)$. The green area represents all the valid positions where $x_2$ can be randomly placed. Particle $x_3$ is obtained as a linear combination between $x_1$ and $x_2$ position vectors. The red point represents the singularity, a point where $x_2$'s and $x_3$'s positions coincide. The axis labels $X_1$ and $X_2$ represent our $x$ and $z$ dimensions respectively. Figure adapted from \citet{Breen2020}.}
        \label{fig:reference_plane}
    \end{figure}

    Particles $x_1$ and $x_3$ positions are quite straightforward to obtain.
    However, particle $x_2$'s position needs to be randomized inside the green area described in Figure~\ref{fig:reference_plane}.
    This means that $x_2$'s position has to be sampled from a uniform distribution, which ensures that the dataset is as diverse and representative as possible.

    To do that, we followed the following process:

    \begin{enumerate}
        \item Sample $\theta \in \left[0, \frac{\pi}{2}\right]$ uniformly;
        \item Create a vector $\left(x, y, z\right)$, whose values are given by:
        \begin{enumerate}
            \item $x = - \min(0.5, \cos(\theta))$
            \item $y = 0$ (this dimension is ignored)
            \item $z = \sin(\theta)$
        \end{enumerate}
        \item Sample $s \in \left[0, 1\right]$ uniformly, and multiply the vector obtained above with this value to calculate the final $x_2$'s position;
    \end{enumerate}

    Next, we used the Brutus integrator~\cite{Boekholt2014} to simulate the motion of the three particles for a total of 10 time units, with a time step of $0.0390625$ time units, which corresponds to a total of 256 time steps per simulation.
    The Brutus integrator also includes two hyperparameters: the word length $L_w$ and the tolerance $\epsilon$, which were set to $88$ and $1.0 \times 10^{-10}$, respectively, following the work of \citet{Breen2020}.

    \todo[inline]{Could be interesting to give a small overview of how Brutus works, and what issues we faced while using it. e.g. the non-converging simulations}

    To make the computation easier, we set the gravitational constant $G$ and the particle's masses to $1$, while their initial velocities were set to $0$ on all dimensions.
    Moreover, the Brutus integrator assumes that the particles' positions and velocities all have 3 dimensions (e.g., $x$, $y$, and $z$), even though we are working on a 2D plane.
    For this reason, we considered only the $x$ and $z$ dimensions in the simulations, while $y$ always remains at $0$.
    Also, the bodies are assumed to be point-particles, meaning that no collision mechanics are to occur during the simulations, even though some very close encounters do happen.

    In total, we generated $30000$ simulations, each with different initial conditions.
    Of these, $26675$ converged numerically (around $88\%$), while the remaining $2325$ did not.
    The non-converging simulations were discarded, and the remaining were used to create our final dataset.
    Figure~\ref{fig:simulations_x2_position_status} shows the distribution of $x_2$'s position for all simulations.

    \begin{figure}[h]
        \centering
        \includegraphics[width=.9\linewidth]{initial_x2_positions_status}
        \caption{Distribution of $x_2$'s position for all simulations. The color represent whether the simulation converged or not. }
        \label{fig:simulations_x2_position_status}
    \end{figure}

    As observed, most non-converging simulations are centered around the singularity point, where $x_2$ and $x_3$ particles are very close to each other.
    This has also been observed in the work of \citet{Breen2020}, where points near the singularity are more likely to have non-converging simulations.

    Additionally, points near the singularity are also more likely to have a higher computational cost, as the Brutus integrator needs to take smaller time steps to ensure the simulation converges.
    Figure~\ref{fig:simulations_x2_position_time} shows the time taken for each simulation to converge.


    \begin{figure}[h]
        \centering
        \includegraphics[width=.9\linewidth]{initial_x2_positions_time_taken}
        \caption{Time taken for each simulation to terminate, whether it converged or not. The color represents the time taken in a logarithmic scale.}
        \label{fig:simulations_x2_position_time}
    \end{figure}

    As observed, the time taken for the simulations to converge is highly dependent on the initial conditions, and points near non-convergence areas are more likely to have a higher computational cost.


    \todo[inline, color=red]{Add figure showing all $x_2$ positions and whether the each simulation converged or not}



    \subsection{Architecture}
    \todo[inline, color=red]{Write the specifics about the architecture}

    We implemented a simple \gls{ANN} for this problem, composed of the following layers [7, 128, 128, 64, 12].

    \subsection{Training Regimen}
    \todo[inline, color=red]{Write out the specifics about the training regimen. This can actually be done right now by taking a look at the training loops, more specific details about specific hyperparameters can be filled in later.}
    
    Therefore, it is straightforward to obtain the positions $\mathbf{p}_1$ and $\mathbf{p}_3$ of the first and third bodies, where any $\mathbf{p}_n \equiv (x_n, y_n = 0, z_n)$ is a three-dimensional spatial vector. However, $\mathbf{p}_2$ must be randomly placed within a defined area while ensuring a uniform sampling of this space to maintain diversity within the dataset. To achieve this, we propose Algorithm \ref{alg:init-cond} to generate meaningful initial positions for the bodies.
    
    \begin{algorithm}[h]
        \caption{Generation of initial conditions for simulation.}
        \label{alg:init-cond}
        \begin{algorithmic}[1]
            \State Sample $\theta$ uniformly from $[0, \frac{\pi}{2}]$.
            \item[]
            \State Create $\mathbf{p} \equiv (x,y,z)$ with the following components:
    
            $x \gets -\min(0.5, \cos(\theta))$
    
            $y \gets 0$ 
    
            $z \gets \sin(\theta)$
            \item[]
            \State Sample $s$ uniformly from $[0, 1]$.
            \State Multiply $\mathbf{p}$ by $s$ to calculate the final position of $p_2$.
        \end{algorithmic}
    \end{algorithm}
    
    Following the generation of the initial positions $\mathbf{p}_{1,2,3}$, the BRUTUS integrator \cite{Boekholt2014} was used to simulate the motions of the three particles for a total of $t = 10$ time units, with a step size of $\Delta t = 0.0390625$, which corresponds to a total of $256$ time steps per simulation. This integration technique is parametrized by two hyperparameters: the word length $L_w$, which corresponds to the bytes used to represent numerical values, and the tolerance $\varepsilon$, which represents the maximum accepted deviation between individual integrators. Following the work of \citet{Breen2020}, these were set to $L_w = 88$ and $\varepsilon = 1.0 \times 10^{-10}$.
    
    As a simplification of the problem, we assumed a unitless system where both the gravitational constant $G$ and the particle masses $m_1 = m_2 = m_3$ were set to $1$. The initial velocities of each particle were assumed to be $0$ across all axes. Additionally, the planar formulation of the three-body problem was adopted, following the methodology of \citet{Breen2020}, which involves assuming constant values for both position and velocity along the $y$-axis. Lastly, the bodies were assumed to be perfectly represented by point particles, ensuring that the probability of collisions is infinitesimally small.
    
    In total, $30000$ simulations unique simulations where generated, of which around $20\%$ did not converge numerically. This divergence occurred mostly when $\mathbf{p}_2$'s position was near the singularity point, where particles $\mathbf{p}_2$ and $\mathbf{p}_3$ are close to each other. Figure \ref{fig:x2-vs-conv} visualizes the distribution of $\mathbf{p}_2$'s position for all simulations and whether they converged.
    
    \begin{figure*}
        \centering
        \begin{subfigure}[t]{0.45\textwidth} %
            \centering
            \includegraphics[width=\textwidth]{initial_x2_positions_status.pdf} %
            \caption{Illustration of the relation between the location of particle $2$ and the convergence of the numerical integrator. Points in blue represent converged simulations, while those in red represent simulations that did not converge.}
            \label{fig:x2-vs-conv}
        \end{subfigure}
        \hfill
        \begin{subfigure}[t]{0.45\textwidth} %
            \centering
            \includegraphics[width=\textwidth]{initial_x2_positions_time_taken.pdf} %
            \caption{Illustration of the relation between the location of particle $2$ and the time to necessary to calculate the full timescale of the simulation.}
            \label{fig:x2-vs-time-taken}
        \end{subfigure}
        \caption{Visualization of the dependence of the BRUTUS three-body simulations on the choice of initial position for particle $2$.}
        \label{fig:x2-vs-multiple}
    \end{figure*}
    \FloatBarrier
    
    

\subsection{Architecture}
\label{subsec:architecture}

    Due to the added constraints introduced by the physics-informed term of the loss, \glspl{PINN} must be more expressive than their counterparts. This increase in expressiveness is achieved by deepening or expanding its width, effectively increasing the number of parameters. In addition to this requirement, the increased complexity of the loss landscape makes PINNs susceptible to the ``exploding gradients problem'', which causes updates to the network to become highly volatile, and eventually destabilizes the training process irreversably \cite{Sharma2023,Bishop2023}. So as to improve gradient flow and possibly avoid this issue, we additionally implemented the ResNet \cite{He2016} architecture. This architecture is similar to a standard feed-forward network, with the addition of residual connections which take the output of layer $l$, and add it to the output of layer $l+n$, visualized in Figure \ref{fig:resnet-block}. 
    
    Given the comparative nature of this study, we have built on the methodology outlined by \citet{Breen2020}. The original author proposed a standard \emph{feed-forward} deep neural network, this is, a network where no closed directed cycles are formed in the neuron graph \cite{Bishop2023}.

    \begin{figure}[h!]
        \centering
        \includegraphics[width=\linewidth]{resnet-block.pdf}
        \caption{Residual block, where $\sigma$ represents any nonlinear activation function and a Fully Connected Linear Layer is a layer of neurons where each is connected to each of the inputs and outputs. A ResNet is composed of successive applications of this block.}
        \label{fig:resnet-block}
    \end{figure}

    Each architecture was additionally formulated under both a non-autoregressive and an autoregressive setup. Firstly, under the non-autoregressive formulation, the model takes as input a 7-vector containing the initial positions of bodies and a time $t_n$, and subsequently predicts a 12-vector representing the state of the system at $t_n$. This output vector is thus composed of both the body positions and velocities. Contrastively, the autoregressive setup takes as input the state of the system at any time $t_0$ and a timestep $\Delta t$, and is tasked with predicting the state of the system at timestep $t = t_0 + \Delta t$.

    As baseline, we have implemented a feed-forward deep neural network composed of 12 layers, each of which may be separated into three categories based on their task: input, hidden and output. A single input layer is used, composed of 7 or 13 units ("neurons"), for non-autoregressive and autoregressive formulations respectively. A total of 10 hidden layers were used, each at a width of 128 units \cite{Breen2020}. Lastly, a single output layer was used composed of 12 units, each responsible for outputting the inferred value associated to an individual variable of the system. Each layer is interspersed with a rectified linear unit (ReLU), a nonlinearity that allows the model to express non-linear functions \cite{Bishop2023}.

    Choices of design for the PINN are discussed in the results section, specifically in Table \ref{tab:hyperparameter-optimization}. 

\subsection{(Physics-Informed) Loss}
\label{subsec:loss}

    As a comparative baseline, we take the loss used by \citet{Breen2020}, this being a mean-absolute-error (MAE) loss, defined by:
    \begin{align}
        \begin{split}
            \mathcal{L}_{\mathrm{MAE}} &= \frac{1}{N_u} \| u(\mathbf{t}_u, \mathbf{x}_u) - \mathbf{u} \|_1\\
            &= \frac{1}{N_u}\sum_{i=1}^{n} |u(t^i_u, x^i_u) - u^i| 
        \end{split}
        \label{eq:pinn-Lu-mae}
    \end{align}
   where we define the set $\{t^i_u, x^i_u, u^i\}^{N_u}_{i=1}$ as the initial data on $u(t,x)$. The MAE loss is thus equivalent to Eq.~\eqref{eq:pinn-Lu}, and serves the purpose of punishing discrepancies between the ground truth and model predictions.

   As priorly mentioned in Section \ref{sec:nn-and-pinn}, physics-informed losses are composed of not only the data discrepancy loss, but also a (partial) differential equation collocation loss that punishes model predictions which do not correspond to the laws of the system, denoted  $\mathcal{L}^{(f)}$, as in Eq. \eqref{eq:pinn-Lf}. 
   
   The total loss of the model may then be defined as
   \begin{equation}
    \mathcal{L} = \mathcal{L}_{\mathrm{MAE}}^{(u)} + \alpha \mathcal{L}^{(f)}
   \end{equation}
   where $\alpha$ is a weighing coefficient attached to the physics-informed loss term. Choice of alpha is discussed in the results section, specifically in Table \ref{tab:hyperparameter-optimization}.

    \subsection{Training Regime}

    According to best practices, the total dataset was partitioned into two sub-sets, a training dataset composed of 95$\%$ of the data used to update the parameters of the model, and a validation set used to verify its ability to generalize \cite{Bishop2023}.

    A model is said to overfit when evaluation on training and validation datasets diverges, favouring the training set, which equates to the model losing generalization capabilities. In order to avoid overfitting, early stopping was implemented, stopping the training process after 10 epochs after the last improvement over the validation set \cite{Prechelt1998}.

    Models were trained using the ADAM \cite{Kingma2017} gradient descent method for a maximum of 500 epochs. In addition, due to the complexity of the loss landscape, learning rate was scheduled to reduce by a factor of $0.7$ in case of a plateau of validation performance lasting 5 epochs.

    Further choices of training regime are further discussed in the results section, specifically under Table \ref{tab:hyperparameter-optimization}.

